Sample Complexity of Uniform Convergence for Multicalibration

There is a growing interest in societal concerns in machine learning systems, especially in fairness. Multicalibration gives a comprehensive methodology to address group fairness. In this work, we address the multicalibration error and decouple it from the prediction error. The importance of decoupling the fairness metric (multicalibration) and the accuracy (prediction error) is due to the inherent trade-off between the two, and the societal decision regarding the "right tradeoff" (as imposed many times by regulators). Our work gives sample complexity bounds for uniform convergence guarantees of multicalibration error, which implies that regardless of the accuracy, we can guarantee that the empirical and (true) multicalibration errors are close. We emphasize that our results: (1) are more general than previous bounds, as they apply to both agnostic and realizable settings, and do not rely on a specific type of algorithm (such as deferentially private), (2) improve over previous multicalibration sample complexity bounds and (3) implies uniform convergence guarantees for the classical calibration error.

==> src/Impact.tex <==
% %Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences.
% % Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss
% %a) who may benefit from this research,
% %b) who may be put at disadvantage from this research,
% %c) what are the consequences of failure of the system, and 
% %d) whether the task/method leverages biases in the data. 
% This work has the following potential positive impact in the society…. At the same time, this work may have some negative consequences because… Furthermore, we should be cautious of the result of failure of the system which could cause...”

The generalization bounds derived in this work can be utilized to measure calibration error of predictors. 
% Verifying that predictors are ``multicalibrated'' provides society with fairness guarantees about their performance. 
% old 8.10 When it comes to predictors that assign probabilities to individuals (e.g., probability of repaying a loan), verifying their fairness have a significant societal impact, and our work makes an important contribution in this matter. 
% We point out that the tools that derive from our work are not applicable for  ``negligible size'' subpopulations 
% (that is, $U\in \Gamma$ such that $\Prob_D[x \in U]<\gamma$).
% At the extreme, we might have subpopulations which are singletons (single individuals), for which one should use individual fairness rather than group fairness.
When it comes to predictors that assign probabilities to individuals (e.g., probability of repaying a loan), verifying that predictors are ``multicalibrated'' provides society with fairness guarantees about their performances.

While our work makes an important contribution to this significant societal matter, we point out some limitations. 
%
First, it is up to regulators to decide upon the subpopulations collection properly. For example, if subpopulations that are characterized by gender are excluded, it might harm major parts of the population.
%
Second, even if the aforementioned issue is tackled, and good approximations for  multicalibration are obtained, they do not dismiss other forms of fairness, and as a result, fairness as a general concept is still not guaranteed.
%
In particular, the tools that derive from our work are not applicable for  ``negligible size'' subpopulations (that is, $U\in \Gamma$ such that $\Prob_D[x \in U]<\gamma$).
At the extreme, we might have subpopulations which are singletons (single individuals), for which one should use individual fairness rather than group fairness.
%
In addition, regulators should use the tools we present with caution as unforeseeable trade-offs between other fairness constraints might also arise, and insuring one form of fairness could lead to worsening others.

Overall, we emphasize that regulators should heavily consider the full meaning of their  choices, and understanding them with respect to multicalibration is only a part of it. 

% %

% In this work, we address the multicalibration error and decouple it from the prediction error.
% %
% The importance of decoupling the fairness metric (multicalibration) and accuracy (prediction error) is due to the inherent trade-off between the two, and the societal decision  regarding %
% the ``right tradeoff'' (as imposed many times by regulators). %

%FROM MEETING There is  [the regulators should understand that while wisiwyg they still have to use our tools carefully, tradeoff between several constraints, .. regulators should worry about fairness. while they can understand the meaning of their choices but they still have to make sure they gurantee fairness. [his responsibilty, to define the subspops and the tradeoff]
% Also- they should define the subpops properly- e.g., without gender.. ]

% account for..

%uniform convergence assures that when working with a bounded complexity predictor class class and there is ``enough data'' and measuring the calibration error of a predictor, then with high probability ``what you see is what you get'' (almost).
%has the following positive impact.
% Namely, given an $(\alpha-\epsilon, \gamma, \psi)$ empirically multicalibrated w.r.t. the data, this predictor is almost certainty an $(\alpha, \gamma, \psi)$–mutlicalibrated with respect to the underlying distribution the data was generated from.  
 

%on their lives, our research yields an evaluation tool for one type of fairness, multicalibration.

%The drawback of this result derives from the notion of fairness itself -- it does not imply fairness guarantees 
% The inherent reason for that lies within the impracticality of acquiring such large datasets, that would achieve this low rates of calibration error.
%For this kind of guarantees, we suggest to use  a different measures of fairness, such as individual fairness \cite{Dwork2012}, and implement other generalization tools.







% Similar to much of the generalization literature in machine learning, our work also concentrates on the statistical aspects of generalization bounds. %, and not algorithmic ones.
% In many cases, the goal might not be to minimize the multicalibration error, but other objectives that depend on the context and the regulator.

% This paper gives society the option to work with any predictor class with bounded complexity, rule-out un-calibrated predictors, and optimize over the remaining calibrated predictors to any desired objective. As we pointed out in the introduction, a multicalibrated predictor does not imply high accuracy. Instead, we prefer to look at a tool that allows to select a multicalibrated predictor among several accurate predictors. 

% Alternatively, if the goal is a multicalibrated predictor, one can simply use the output predictor from running an empirical multicalibration risk minimization over a hypothesis class with bounded complexity $\HH$. By uniform convergence, a similar true multicalibraion error is guaranteed. Unfortunately, without realizability, it is known to be an NP-hard problem even for such a relatively simple class of functions as linear classifiers \cite{Feldman2009}.


% % There is a vast difference between multicalibration uniform convergence and multicalibrated predictors:
% % Having a uniform convergence property implies that the empirical and true errors are similar, but does not imply that they are low. Also, having a predictor with zero multicalibration error (realizability) does not imply anything about the generalization error.  




